Spatial Principal Component Analysis and Moran Statistics for Multivariate Functional Areal Data

The paper introduces a multivariate functional areal spatial principal component analysis (mfasPCA) framework, together with multivariate functional Moran's I statistics, to enable the assessment of spatial autocorrelation and dimension reduction for multivariate functional data observed over areal units. The proposed framework is spatial-functional in scope: the functional argument may represent time, age, wavelength, or another ordered continuum, while spatial dependence is introduced across areal units through a spatial weight matrix. The principal component method is defined through a Moran-type spatially weighted criterion. We propose eigenvalue-based permutation tests to assess the significance of spatially structured components. The testing framework includes omnibus tests, componentwise tests with Holm adjustment, and sequential rank-wise tests based on tail sums of eigenvalues. Simulation studies show that mfasPCA captures positive and negative spatial-functional structures and concentrates them in the leading components under the respective autocorrelation regimes. A real-data application illustrates how mfasPCA identifies spatially structured modes of multivariate functional variation.

==> preamble.tex <==
%% =====================================================================
%% preamble.tex
%% =====================================================================

%% --- Page & encoding ---
\usepackage[margin=1in]{geometry}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{lmodern}
% \usepackage{microtype}
\usepackage[english]{babel} % american english
\usepackage{comment}
\usepackage{setspace}

%% --- Math ---
\usepackage{amsmath,amsthm,amsfonts,amssymb,mathtools}

%% --- Figures & graphics ---
\usepackage{graphicx}
\usepackage[dvipsnames]{xcolor}
\usepackage{adjustbox}
\usepackage{float}

%% --- Captions & subfigures (order matters) ---
\usepackage{caption}
\usepackage{subcaption}

\captionsetup[table]{justification=raggedright, singlelinecheck=false, labelsep=quad, width=\textwidth, labelfont=bf, font=small}
\captionsetup[figure]{name=Fig., labelsep=quad, width=\textwidth, labelfont=bf}

%% --- Tables ---
\usepackage{array}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage{threeparttable}
\usepackage{dcolumn,tabularx}

\newcolumntype{d}[1]{D{.}{.}{#1}}  % define "d" column type
\newcommand\mc[1]{\multicolumn{1}{c}{#1}} % handy shortcut macro

%% --- Utilities ---
\usepackage{placeins}    % \FloatBarrier
\usepackage{pdfpages}
\usepackage[hidelinks]{hyperref}
\usepackage{natbib}

\providecommand{\bibcommenthead}{}

%% --- Blank placeholder for missing images (auto-remap) ---
\usepackage{ifthen}
\makeatletter
\let\OrigIncludeGraphics\includegraphics
\newcommand{\blankinclude}[2][]{%
  \IfFileExists{#2}{%
    \OrigIncludeGraphics[#1]{#2}%
  }{%
    \begingroup
      \setkeys{Gin}{#1}%
      \ifdim\Gin@req@width=0pt \Gin@req@width=4cm\fi
      \ifdim\Gin@req@height=0pt \Gin@req@height=6cm\fi
      \setlength{\fboxsep}{0pt}%
      \framebox[\Gin@req@width][c]{\rule{0pt}{\Gin@req@height}}%
    \endgroup
  }%
}
\renewcommand{\includegraphics}[2][]{\blankinclude[#1]{#2}}
\makeatother

%% ---- K_USE per-weight macros (default shows the symbolic form) ----
\newcommand{\Kuse}{K_{\text{USE}}}
\newcommand{\KuseSym}{$K_{\text{USE}}$}
\newcommand{\KuseWone}{\KuseSym}   % W1: knn standard
\newcommand{\KuseWtwo}{\KuseSym}   % W2: knn symmetric
\newcommand{\KuseWthree}{\KuseSym} % W3: radial
\newcommand{\KuseWfour}{\KuseSym}  % W4: power
\newcommand{\KuseWfive}{\KuseSym}  % W5: exponential
\newcommand{\KuseWsix}{\KuseSym}   % W6: double-power
\newcommand{\KuseWseven}{\KuseSym} % W7: rook
\newcommand{\KuseWeight}{\KuseSym} % W8: shared-boundary
\newcommand{\KuseWnine}{\KuseSym}  % W9: combined

%% ---- Sections & subsections, tables & figures numbering ----
\renewcommand{\thesection}{\Alph{section}}
\renewcommand{\thesubsection}{\thesection.\arabic{subsection}}

\numberwithin{figure}{section}
\numberwithin{table}{section}

\renewcommand{\thefigure}{\thesection\arabic{figure}}
\renewcommand{\thetable}{\thesection\arabic{table}}

